Sharing tea on a graph

Motivated by the analysis of consensus formation in the Deffuant model for social interaction, we consider the following procedure on a graph $G$. Initially, there is one unit of tea at a fixed vertex $r \in V(G)$, and all other vertices have no tea. At any time in the procedure, we can choose a connected subset of vertices $T$ and equalize the amount of tea among vertices in $T$. We prove that if $x \in V(G)$ is at distance $d$ from $r$, then $x$ will have at most $\frac{1}{d+1}$ units of tea during any step of the procedure. This bound is best possible and answers a question of Gantert. We also consider arbitrary initial weight distributions. For every finite graph $G$ and $w \in \mathbb{R}_{\geq 0}^{V(G)}$, we prove that the set of weight distributions reachable from $w$ is a compact subset of $\mathbb{R}_{\geq 0}^{V(G)}$.

==> _preamble/myBiblatex.tex <==

\usepackage[
    style=ieee,
    sorting=nyt,
    uniquename=init,
    defernumbers=true,
    maxnames=12,
    isbn=false,
    dashed=false,
    giveninits=false,
    datamodel=_preamble/mrnumber,
]{biblatex}


\RequirePackage{csquotes}
\RequirePackage{xpatch}
\RequirePackage{xstring}
\RequirePackage[fixed]{fontawesome5}

\newcommand{\linksymbol}{\scalebox{0.75}{\textcolor{black!75}{\faLink}}}


    \DeclareFieldFormat[article]{title}{``#1''}
    \DeclareFieldFormat[article]{volume}{\addnbspace\textbf{#1}}
    \DeclareFieldFormat[article]{number}{(#1)}
    \DeclareFieldFormat[article]{pages}{%
    \IfSubStr{#1}{Paper}{,\addnbspace#1}{:#1}}%
    
    \DeclareFieldFormat[article,book,incollection,inproceedings]{url}{%
        \linksymbol \href{#1}{#1}}
    \DeclareFieldFormat[article,book,incollection,inproceedings]{doi}{%
        \linksymbol \href{https://doi.org/#1}{DOI: #1}}
    \DeclareFieldFormat[article,book,incollection,inproceedings]{eprint:arxiv}{%
        \linksymbol \href{https://arxiv.org/abs/#1}{arXiv: #1}}
    \DeclareFieldFormat[article,book,incollection,inproceedings]{mrnumber}{%
        \linksymbol \href{http://www.ams.org/mathscinet-getitem?mr=#1}{MR: #1}}

    \DeclareBibliographyDriver{article}{%
        \usebibmacro{bibindex}%
        \usebibmacro{begentry}%
        \textsc{\usebibmacro{author/translator+others}}%
        \newunit
        \usebibmacro{title}%
        \newunit
        \printlist{language}%
        \newunit\newblock
        \usebibmacro{byauthor}%
        \newunit\newblock
        \usebibmacro{bytranslator+others}%
        \newunit\newblock
        \printfield{version}%
        \newunit\newblock
        \usebibmacro{journal}%
        \printfield{volume}%
        \printfield{number}%
        \printfield{pages}%
        \newunit
        \usebibmacro{date}%
        \newunit
        \printfield{note}%
        \newunit\newblock
        \usebibmacro{addendum+pubstate}%
        \setunit{\bibpagerefpunct}\newblock
        \usebibmacro{pageref}%
        \newunit\newblock
        \iftoggle{bbx:related}
            {\usebibmacro{related:init}%
             \usebibmacro{related}}
            {}%
        \newunit\newblock
        \usebibmacro{finentry}
        \iftoggle{linklinebreak}{\newline}{}
        \iffieldundef{url}{}{\printfield{url}\addspace}%
        \iffieldundef{doi}{}{\printfield{doi}\addspace}%
        \iffieldundef{eprint}{}{\usebibmacro{eprint}\addspace}%
        \iffieldundef{mrnumber}{}{\printfield{mrnumber}\addspace}}

    
    \DeclareBibliographyDriver{book}{%
        \usebibmacro{bibindex}%
        \usebibmacro{begentry}%
        \textsc{\usebibmacro{author/editor+others/translator+others}}%
        \setunit{\labelnamepunct}\newblock
        \usebibmacro{maintitle+title}%
        \usebibmacro{series+number(book)}%
        \printlist{language}%
        \newunit\newblock
        \printfield{edition}%
        \newunit\newblock
        \usebibmacro{byauthor}%
        \newunit\newblock
        \usebibmacro{byeditor+others}%
        \newunit\newblock
        \printfield{volumes}%
        \newunit\newblock
        \setunit{\adddot\addspace}%
        \newblock
        \usebibmacro{publisher+location+date}%
        \newunit\newblock
        \usebibmacro{volume+part}%
        % \newunit
        % \usebibmacro{chapter+pages}%
        % \newunit
        % \printfield{pagetotal}%
        \newunit\newblock
        \printfield{note}%
        \newunit\newblock
        \iftoggle{bbx:isbn}
         {\printfield{isbn}}
         {}%
        % \newunit\newblock
        % \usebibmacro{doi+eprint+url}%
        \newunit\newblock
        \usebibmacro{addendum+pubstate}%
        \setunit{\bibpagerefpunct}\newblock
        \usebibmacro{pageref}%
        \newunit\newblock
        \iftoggle{bbx:related}
         {\usebibmacro{related:init}%
          \usebibmacro{related}}
         {}%
        \usebibmacro{finentry}
        \iftoggle{linklinebreak}{\newline}{}
        \iffieldundef{url}{}{\printfield{url}\addspace}%
        \iffieldundef{doi}{}{\printfield{doi}\addspace}%
        \iffieldundef{eprint}{}{\usebibmacro{eprint}\addspace}%
        \iffieldundef{mrnumber}{}{\printfield{mrnumber}\addspace}}

        
    \DeclareBibliographyDriver{incollection}{%
        \usebibmacro{bibindex}%
        \usebibmacro{begentry}%
        \textsc{\usebibmacro{author/translator+others}}%
        \setunit{\labelnamepunct}\newblock
        \usebibmacro{title}%
        \newunit
        \printlist{language}%
        \newunit\newblock
        \usebibmacro{byauthor}%
        \newunit\newblock
        \usebibmacro{in:}%
        \usebibmacro{maintitle+booktitle}%
        \newunit\newblock
        \usebibmacro{series+number}%
        \newunit\newblock
        \usebibmacro{byeditor+others}%
        \newunit\newblock
        \printfield{edition}%
        \newunit
        \iffieldundef{maintitle}
         {\printfield{volume}%
          \printfield{part}}
         {}%
        \newunit
        \printfield{volumes}%
        \newunit\newblock
        \printfield{note}%
        \newunit\newblock
        \usebibmacro{chapter+pages}%
        \newunit\newblock
        \usebibmacro{publisher+location+date}%
        \newunit\newblock
        \iftoggle{bbx:isbn}
         {\printfield{isbn}}
         {}%
        % \newunit\newblock
        % \usebibmacro{doi+eprint+url}%
        \newunit\newblock
        \usebibmacro{addendum+pubstate}%
        \setunit{\bibpagerefpunct}\newblock
        \usebibmacro{pageref}%
        \newunit\newblock
        \iftoggle{bbx:related}
         {\usebibmacro{related:init}%
          \usebibmacro{related}}
         {}%
        \usebibmacro{finentry}
        \iftoggle{linklinebreak}{\newline}{}
        \iffieldundef{url}{}{\printfield{url}\addspace}%
        \iffieldundef{doi}{}{\printfield{doi}\addspace}%
        \iffieldundef{eprint}{}{\usebibmacro{eprint}\addspace}%
        \iffieldundef{mrnumber}{}{\printfield{mrnumber}\addspace}}

    \DeclareBibliographyDriver{inproceedings}{%
        \usebibmacro{bibindex}%
        \usebibmacro{begentry}%
        \textsc{\usebibmacro{author/translator+others}}%
        \setunit{\labelnamepunct}\newblock
        \usebibmacro{title}%
        \newunit
        \printlist{language}%
        \newunit\newblock
        \usebibmacro{byauthor}%
        \newunit\newblock
        \usebibmacro{maintitle+booktitle(inproceedings)}%
        \midsentence
        \newunit\newblock
        \usebibmacro{event+venue+date}%
        \newunit\newblock
        \usebibmacro{byeditor+others}%
        \newunit\newblock
        \printfield{volumes}%
        \newunit\newblock
        \usebibmacro{series+number}%
        \newunit\newblock
        \printfield{note}%
        \newunit\newblock
        \printlist{organization}%
        \newunit\newblock
        \usebibmacro{volume+part}%
        \newunit\newblock
        \usebibmacro{chapter+pages}%
        \newunit
        \usebibmacro{publisher+location+date}%
        \newunit\newblock
        \iftoggle{bbx:isbn}
         {\printfield{isbn}}
         {}%
        % \newunit\newblock
        % \usebibmacro{doi+eprint+url}%
        \newunit\newblock
        \usebibmacro{addendum+pubstate}%
        \setunit{\bibpagerefpunct}\newblock
        \usebibmacro{pageref}%
        \newunit\newblock
        \iftoggle{bbx:related}
        {\usebibmacro{related:init}%
          \usebibmacro{related}}
         {}%
        \usebibmacro{finentry}
        \iftoggle{linklinebreak}{\newline}{}
        \iffieldundef{url}{}{\printfield{url}\addspace}%
        \iffieldundef{doi}{}{\printfield{doi}\addspace}%
        \iffieldundef{eprint}{}{\usebibmacro{eprint}\addspace}%
        \iffieldundef{mrnumber}{}{\printfield{mrnumber}\addspace}}


\newtoggle{linklinebreak}
\AtEveryBibitem{%
    \iffieldundef{doi}{%
        \iffieldundef{url}{%
            \iffieldundef{eprint}{%
                \iffieldundef{mrnumber}{
                    \togglefalse{linklinebreak}%
                }{\toggletrue{linklinebreak}}
            }{\toggletrue{linklinebreak}}%
        }{\toggletrue{linklinebreak}}%
    }{\clearfield{url}\toggletrue{linklinebreak}}}

\renewcommand{\bibfont}{\scriptsize}
% \setlength{\bibitemsep}{1pt}
% \setlength{\bibhang}{2.5em}
% \xpretofieldformat{doi}
%   {\newline\linksymbol}
%   {}{}
% \xpretofieldformat{url}
%   {\newline\linksymbol}
%   {}{}
% \xpretofieldformat{eprint:arxiv}
%   {\iftoggle{linklinebreak}{\linksymbol}{\newline\linksymbol}}
%   {}{}
% \xpretofieldformat{mrnumber}
%   {\iftoggle{linklinebreak}{\linksymbol}{\newline\linksymbol}}
%   {}{}

